Catalog of Integrated-Light Star Cluster Light Curves in TESS

We present the first integrated light, TESS-based light curves for star clusters in the Milky Way, Small Magellanic Cloud, and Large Magellanic Cloud. We explore the information encoded in these light curves, with particular emphasis on variability. We describe our publicly available package ELK, which is designed to extract the light curves by applying principal component analysis to perform background light correction, and incorporating corrections for TESS systematics, allowing us to detect variability on time scales shorter than ~10 days. We perform a series of checks to ensure the quality of our light curves, removing observations where systematics are identified as dominant features, and deliver light curves for 348 previously-cataloged open and globular clusters. Where TESS has observed a cluster in more than one observing sectors, we provide separate light curves for each sector (for a total of 2204 light curves). We explore in detail the light curves of star clusters known to contain high-amplitude Cepheid and RR Lyrae variable stars, and confirm that the variability of these known variables is still detectable when summed together with the light from thousands of other stars. We also demonstrate that even some low-amplitude stellar variability is preserved when integrating over a stellar population.

==> Referee_Report.tex <==
Overall:

In this work, the authors present a TESS data pipeline for - and subsequent study of - integrated TESS light curves of clusters in the Milky Way, the SMC and the LMC. They explore whether stellar signals from known individual variable star sources are retained in the periodograms of the integrated light curves, and through simulations explore how much cluster information is maintained in the integrated light. They also publish the catalogue of their extracted light curves, along with an open-source Python package used to make the extractions. The paper is concise and well written, and covers the relevant background and references to the literature.

Below are comments on the content which I think require addressing before publication - but all of these are requests for additional information to be included in the text or provided in the response to the reviewer, and none will require additional analysis to be performed. There are also some minor comments which do not need addressing or commenting on, but which I hope will provide useful feedback to the authors. I very much enjoyed reading the paper.


Primary comments:

%Done
Line 219: "..has the added benefit of preferentially selecting clusters with relatively smaller amounts of non-member contamination."
This wording implies that not having non-member contamination is a property of the clusters (which in turn implies something about distance and location), not a property of the selection effect. If I understand this correctly, what instead happens here is that the maximum radius reduction will reduce the non-member contamination, at the risk of also excluding true member stars.
    Reply: We agree this sentence was ambiguous, and have rephrased in the text.

%Done
Line 358: Here the authors state that they build a model with components that include the TESS mission CBVs from the SPOC pipeline. In the Data section, they state that the data from the FFIs have been processed by the SPOC pipeline already. Figure 2, shows that the CBV components from SPOC are essential in removing the systematics, so I'm a bit confused about what's going on. If the authors are applying the CBVs from the SPOC pipeline to data that has already been detrended by SPOC, aren't they doubling up on the correction here?
    Reply: We have clarified this by specifying the data comes from the SPOC 'FFI' pipeline, which does not incorporate CBVs. We have also expanded the sentence describing SPOC to say that it provides "supplemental products for additional systematic correction", specifying that the CBVs are additional to the processing done by the pipeline. 

%Done
Line 363 - 415: I think the authors may already do so later in the text, but I think it is important to explain why they make the selection at 10 days at this first mention of it, instead. It may be that when looking at the detrended data the long period trends are still difficult to measure (I know the field as a whole is struggling with this) - but for an outside reader looking in they may be surprised that the introduction of the CBVs, which are stated to capture variability common across the CCD, do not account for the 15 day orbital systematic.
    Reply: We have moved the paragraph from the end of the subsection describing the 10 day selection to immediately follow this paragraph where we first mention the 10 day selection.  

%Done
Line 378-384: Can the authors please expand on how you determined the optimum number of PCA components? Or if it is fully covered by the sentence from lines 381, 384, maybe clarify that they found this threshold of 6 components to apply equally to all clusters. 
    Reply: These lines encompass the test we performed to determine the optimal number of PCA components. The test suite of clusters is representative for clusters in the catalog in terms of their background stellar density and scattered light intensity, and the "best" number of PCA components was consistent across the suite. We have added clarification to the text that this number was chosen from studying a subset of the full catalog. 

%Done
Line 387: Please define the variables mu and sigma.
    Reply: We have defined the variables, and clarified that these are specific parameter settings within the lightkurve package. 

%Done
Line 409: "...preserves the stellar signal"
Is it possible to quantify the noise floor above which stellar signal is preserved? I think this is important information given the nature of the work (in particular the exploration of how well individual stellar signals are preserved when the light is integrated across a cluster).
    Reply: This is a very good point. We thank the referee for bringing up this issue, and think this will add value to the paper. The answer is complex, and not easily quantifiable, since it depends on the specific details of the stellar signal. We performed 2 tests to attempt to answer this question. The first is a K-S test for a synthetic cluster light curve and a bootstrap sampled light curve with decreasing SNR. While the K-S test is a measurement of the overall flux distribution, and not the features in a light curve, this test does indicate that the SNR needed to change the flux distribution is significantly higher than the SNR in our measurements. We added a paragraph to Section 4.1 (where we discuss SNR) describing this test and the results. 
    
    The second test addresses the recovery of a single stellar signal. Here, we test at what SNR the signal from a single source is no longer detectable in the LSP. We chose to perform this test for the Cepheid DL Cas in NGC 129. Our elk code can recover the signal for SNR greater that 35, well below that of our clusters in our catalog. We have added a paragraph to Section 5.3 (where we discuss NGC 129) to describe the test and the results. 

%Done
Line 454: Were adjacent sector light curves combined for the purposes of this analysis? Why/why not?
    Reply: Each sector light curve is presented independently. We explore the impacts of sector stitching in Section 5.2, and encourage users to do this if the data is available, but do not provide sector stitched light curves as a part of the catalog. The typical format for TESS light curve available on MAST is a single sector, and we kept with that format. Because each of our light curves will be available on MAST, anyone who wants to perform sector stitching is welcome to do so.

%Done
Line 611: I'm confused as to why the other 20 RRLs mentioned are not explored further in the text and/or figure, or would this make the plot too busy?
    Reply: We did assess the recovery of the other 20 RRLs. Since the purpose for this subsection is to demonstrate the analysis method is reliable, we specifically highlight 2 RRL stars in this section as the proof of concept for the tool, and dedicate Section 5.2 to analyzing a fuller set of RRL in a cluster. We address the other RRLs briefly in the text, and state there are other features in the LSP which can be traced back to these RRL stars. The referee is correct that Figure 5 would be very busy and hard to read with many additional lines. 

%Done
Line 647: If I'm understanding this correctly, one of the aims of this work is to explore how integrated light curves can contain information from astrophysical sources by comparing integrated TESS light curves to known information of stars contained within the aperture. The example considered in Figure 5 and the accompanying text discusses clear astrophysical signal, but in these cases all three signals occur in the fringes of the cluster. Is the signal contribution of these three targets, which are not as subject to crowding as the core cluster stars, truly analogous to signal contributions from stars in the more crowded core? I'm bringing this up since other clusters may only be contained in a couple of TESS pixels (for example, the cluster shown in Figure 6), and so I want to confirm whether the analysis presented in Figure 5 can be appropriately applied to such targets.
    Reply: This point is well made, and we address it in an updated Figure 6. We have added points to the middle panel of Figure 6 indicating where the RRLs are located and some text in the section to highlight their distribution. NGC 1261 is the better candidate to address crowding as this Section fully explores each RRL with an existing spatial flux map, and shows each RRL star is recovered.  
    

%Done
Line 1028: This is pedantic, but: "...stellar variability information of the stars in the cluster" - I think "some stars in the cluster" or "a number of stars in the cluster" is more appropriate. No way of knowing whether the authors are seeing all the available information of the stars.
    Reply: We have updated the text to reflect this change. 



Minor comments (address at authors' discression, just thoughts and/or advice):

%Done
Introduction, lines 109 - 146: I think the authors cover all necessary citations and background information which is why this is a minor comment, but I think the flow and narrative of this passage could be improved somewhat. Reading it, it is not immediately obvious to me what the value is of doing photometry with integrated light. Placing emphasis on "calibrating" integrated light photometry through comparison to resolved photometry of the same objects (as done later in this paper) would provide a better introductory foothold to the value of your work.
    Reply: Thank you for this comment. We certainly didn't intend to argue that integrated light is superior, just that it's necessary for the foreseeable future. We have added 2 sentences to highlight that while not optimal, integrated light photometry is the only option for systems where individual stars cannot be resolves, and therefore we must enhance our integrated light analysis techniques.

%Done
Cluster Light Curves, 336: There is inconsistency in the name Tesscut (in some places its TESScut, in others its \texttt{TESS-CUT}.
    Reply: This has been corrected. 

%Done
Line 452: Using an average to mention how many sectors were observed feels wrong to me for something that can only be expressed in integers... reporting the mode may be more appropriate.
    Reply: This point is well made. We have changed to the median to match the previous section.

%Done
Line 489: Is it perhaps possible to comment on why these clusters do not pass the authors' quality checks?
    Reply: We have added a sentence detailing how the majority failed the scattered light test, and some failed a combination of tests.

%Done
Line 579: "Therefore, we can investigate how the variability ... correlates with known individual ... observations"
This is a big deal and I don't think its pointed out in the introduction, unless I'm mistaken. Mentioning it there would help sell the paper.
    Reply: Thank you for this comment. We have added a sentence to the introduction to address this point.

Line 954-959: Based on the content of the previous section, I think I'd actually disagree with the emphasis on the power of individual stars here - as the simulation analysis here shows that it's the ensemble properties of the population that provide the interesting information.
    Reply: We have added a sentence to the paragraph highlighting the impact of the stellar ensemble. 

%Done
Line 1024: Is arbitrary the right word here? The apertures are clearly defined based on criteria you set out.
    Reply: This sentence is attempting to relay that the elk code is not only applicable to clusters, but for any defined aperture. We have changed this word to be to "a given". 

---

Data Editor's review :

One of our data editors has reviewed your initial manuscript submission and has the following suggestion(s) to help improve the data, software citation and/or overall content. Please treat this as you would a reviewer's comments and respond accordingly in your report to the science editor. Questions can be sent directly to the data editors at data-editors@aas.org.

It is great that the authors have minted a DOI for the MAST data used in their article. The next step is to include this DOI in the revised manuscript. Ideally, the authors should use the AASTeX "\dataset" command to mark up the DOI so it can be properly tagged in production. An example would be text similar to this:

"The all sector TESS Raw Full Frame Image data presented in this paper were obtained from the Mikulski Archive for Space Telescopes (MAST) at the Space Telescope Science Institute. The specific observations analyzed can be accessed via \dataset[DOI: 10.17909/3y7c-wa45]{https://doi.org/10.17909/3y7c-wa45}.

Ideally, the authors should get MAST to mint a DOI for the HLSP that will host their lightcurves and include this DOI in the revised manuscript like the TESS all sector DOI above. 

    Reply: We have obtained a DOI for MAST for our light curves, which is now included in the text. We have also added the DOI for the FFI data. 

==> Tables/LMC_for_paper.tex <==
\begin{table}
\begin{tabular}{ccccccccccc}
name & Ra [deg] & Dec [deg] & radius [deg] & log_age & n_obs & n_good_obs & which_sectors_good & lc_lens & normalized_stdev & normalized_range \\
NGC1652 & 69.59167 & -68.6725 & 0.01 & 8.5 & 26 & 15 & ['TMS-2', 'TMS-3', 'TMS-9', 'TMS-11', 'TMS-12', 'TMS-13', 'TMS-27', 'TMS-28', 'TMS-29', 'TMS-30', 'TMS-31', 'TMS-33', 'TMS-37', 'TMS-38', 'TMS-39'] & [1196, 1077, 1084, 1180, 1234, 1283, 3351, 3449, 3572, 3681, 3445, 3485, 3461, 3693, 3865] & ['0.000515', '0.000545', '0.000544', '0.001179', '0.000643', '0.000501', '0.000854', '0.000835', '0.000765', '0.000766', '0.001975', '0.001073', '0.00069', '0.000778', '0.000915'] & ['0.001688', '0.001725', '0.001736', '0.001206', '0.001667', '0.001581', '0.002746', '0.002714', '0.002449', '0.002429', '0.006203', '0.00354', '0.001956', '0.002535', '0.002884'] \\
[SL63] 37 & 71.69167 & -72.39472 & 0.02 & 8.7 & 28 & 17 & ['TMS-2', 'TMS-3', 'TMS-7', 'TMS-9', 'TMS-10', 'TMS-11', 'TMS-12', 'TMS-13', 'TMS-27', 'TMS-28', 'TMS-29', 'TMS-30', 'TMS-37', 'TMS-38', 'TMS-39', 'TMS-61', 'TMS-62'] & [1196, 1077, 1086, 1084, 1150, 1180, 1234, 1283, 3351, 3449, 3572, 3681, 3461, 3693, 3865, 10653, 10811] & ['0.000382', '0.000457', '0.001728', '0.000412', '0.000484', '0.000536', '0.000428', '0.000384', '0.000711', '0.000661', '0.000604', '0.000604', '0.000643', '0.000671', '0.000705', '0.0009', '0.001006'] & ['0.001265', '0.001408', '0.003991', '0.001322', '0.001047', '0.001142', '0.001193', '0.001239', '0.002359', '0.002087', '0.001922', '0.00188', '0.002004', '0.002195', '0.002337', '0.002385', '0.002909'] \\
NGC1695 & 71.93333 & -69.37389 & 0.01 & 8.0 & 30 & 17 & ['TMS-2', 'TMS-3', 'TMS-4', 'TMS-9', 'TMS-10', 'TMS-11', 'TMS-12', 'TMS-13', 'TMS-27', 'TMS-28', 'TMS-29', 'TMS-30', 'TMS-33', 'TMS-38', 'TMS-39', 'TMS-63', 'TMS-64'] & [1196, 1077, 1027, 1084, 1150, 1180, 1234, 1283, 3351, 3449, 3572, 3681, 3485, 3693, 3865, 10942, 11276] & ['0.000492', '0.000646', '0.000556', '0.000518', '0.000434', '0.000428', '0.000518', '0.000527', '0.000683', '0.000703', '0.000676', '0.000692', '0.002112', '0.000733', '0.000787', '0.001263', '0.001303'] & ['0.001669', '0.00171', '0.001799', '0.001659', '0.001214', '0.001225', '0.001436', '0.00162', '0.002213', '0.00232', '0.002202', '0.002226', '0.006703', '0.002399', '0.002562', '0.004167', '0.004286'] \\
NGC1698 & 72.26667 & -69.11472 & 0.01 & 8.0 & 29 & 23 & ['TMS-2', 'TMS-3', 'TMS-4', 'TMS-6', 'TMS-7', 'TMS-9', 'TMS-10', 'TMS-11', 'TMS-12', 'TMS-13', 'TMS-27', 'TMS-28', 'TMS-29', 'TMS-30', 'TMS-31', 'TMS-32', 'TMS-33', 'TMS-36', 'TMS-37', 'TMS-38', 'TMS-39', 'TMS-61', 'TMS-63'] & [1196, 1077, 1027, 980, 1086, 1084, 1150, 1180, 1234, 1283, 3351, 3449, 3572, 3681, 3445, 3589, 3485, 3467, 3461, 3693, 3865, 10653, 10942] & ['0.001776', '0.004937', '0.004642', '0.003336', '0.004123', '0.000866', '0.002136', '0.004366', '0.002669', '0.004369', '0.003165', '0.005135', '0.001602', '0.004683', '0.003841', '0.004356', '0.00376', '0.003393', '0.004557', '0.004253', '0.003071', '0.003282', '0.005548'] & ['0.005842', '0.017143', '0.017566', '0.010088', '0.015588', '0.002163', '0.007172', '0.015609', '0.00939', '0.016016', '0.010123', '0.018844', '0.004948', '0.016373', '0.012348', '0.016969', '0.012077', '0.012153', '0.017114', '0.014814', '0.009098', '0.010482', '0.018627'] \\
NGC1704 & 72.47917 & -69.75528 & 0.01 & 7.5 & 29 & 18 & ['TMS-3', 'TMS-5', 'TMS-6', 'TMS-7', 'TMS-9', 'TMS-10', 'TMS-13', 'TMS-27', 'TMS-28', 'TMS-30', 'TMS-31', 'TMS-32', 'TMS-33', 'TMS-37', 'TMS-39', 'TMS-61', 'TMS-63', 'TMS-64'] & [1077, 1176, 980, 1086, 1084, 1150, 1283, 3351, 3449, 3681, 3445, 3589, 3485, 3461, 3865, 10653, 10942, 11276] & ['0.002961', '0.00437', '0.002454', '0.001423', '0.001187', '0.005299', '0.007105', '0.003966', '0.003997', '0.0056', '0.004388', '0.007002', '0.007448', '0.005308', '0.006323', '0.004429', '0.007397', '0.006699'] & ['0.005152', '0.01412', '0.006831', '0.003203', '0.00205', '0.002672', '0.022258', '0.013081', '0.007731', '0.01799', '0.014087', '0.021389', '0.020891', '0.019322', '0.021566', '0.01586', '0.023591', '0.019883'] \\
\end{tabular}
\end{table}


==> Tables/MW_for_paper.tex <==
\begin{table}
\begin{tabular}{ccccccccccc}
name & Ra [deg] & Dec [deg] & radius [deg] & log_age & n_obs & n_good_obs & which_sectors_good & lc_lens & normalized_stdev & normalized_range \\
ASCC 116 & 329.625 & 54.49 & 0.14 & 7.95 & 4 & 4 & ['TMS-16', 'TMS-17', 'TMS-56', 'TMS-57'] & [935, 1126, 11766, 10791] & ['0.000621', '0.000704', '0.00068', '0.000855'] & ['0.002056', '0.002352', '0.002213', '0.002745'] \\
ASCC 57 & 152.73 & -66.7 & 0.215 & 9.26 & 6 & 3 & ['TMS-11', 'TMS-36', 'TMS-38'] & [1180, 3467, 3693] & ['0.000182', '0.000218', '0.000216'] & ['0.000598', '0.000719', '0.000713'] \\
ASCC 8 & 35.19 & 59.69 & 0.24 & 7.77 & 2 & 2 & ['TMS-18', 'TMS-58'] & [1103, 11692] & ['0.000214', '0.000162'] & ['0.00057', '0.000534'] \\
ASCC 81 & 236.692 & -50.995 & 0.16 & 8.75 & 2 & 2 & ['TMS-12', 'TMS-39'] & [1234, 3865] & ['0.000373', '0.000649'] & ['0.001216', '0.002036'] \\
ASCC 9 & 41.745 & 57.745 & 0.21 & 7.0 & 2 & 1 & ['TMS-18'] & [1103] & ['0.000906'] & ['0.002909'] \\
\end{tabular}
\end{table}


==> Tables/SMC_for_paper.tex <==
\begin{table}
\begin{tabular}{ccccccccccc}
name & Ra [deg] & Dec [deg] & radius [deg] & log_age & n_obs & n_good_obs & which_sectors_good & lc_lens & normalized_stdev & normalized_range \\
OGLE-CL SMC  324 & 6.18083 & -73.75389 & 0.03 & 9.15 & 4 & 2 & ['TMS-27', 'TMS-28'] & [3351, 3449] & ['0.000481', '0.000508'] & ['0.001557', '0.00158'] \\
OGLE-CL SMC  319 & 6.19167 & -72.79389 & 0.06 & 9.81 & 3 & 2 & ['TMS-27', 'TMS-28'] & [3351, 3449] & ['0.000253', '0.000276'] & ['0.000814', '0.000901'] \\
OGLE-CL SMC  311 & 6.70208 & -71.53472 & 0.06 & 10.02 & 3 & 2 & ['TMS-27', 'TMS-28'] & [3351, 3449] & ['0.000287', '0.000239'] & ['0.000906', '0.000774'] \\
NGC152 & 8.23458 & -73.11583 & 0.05 & 9.09 & 3 & 2 & ['TMS-27', 'TMS-28'] & [3351, 3449] & ['0.000301', '0.000264'] & ['0.000978', '0.000866'] \\
HW8 & 8.445 & -73.63278 & 0.03 & 8.0 & 4 & 2 & ['TMS-27', 'TMS-28'] & [3351, 3449] & ['0.000662', '0.000637'] & ['0.002163', '0.002117'] \\
\end{tabular}
\end{table}

